DoseRAD2026 Challenge dataset: AI accelerated photon and proton dose calculation for radiotherapy

Purpose: Accurate dose calculation is essential in radiotherapy for precise tumor irradiation while sparing healthy tissue. With the growing adoption of MRI-guided and real-time adaptive radiotherapy, fast and accurate dose calculation on CT and MRI is increasingly needed. The DoseRAD2026 dataset and challenge provide a public benchmark of paired CT and MRI data with beam-level photon and proton Monte Carlo dose distributions for developing and evaluating advanced dose calculation methods. Acquisition and validation methods: The dataset comprises paired CT and MRI from 115 patients (75 training, 40 testing) treated on an MRI-linac for thoracic or abdominal lesions, derived from the SynthRAD2025 dataset. Pre-processing included deformable image registration, air-cavity correction, and resampling. Ground-truth photon (6 MV) and proton dose distributions were computed using open-source Monte Carlo algorithms, yielding 40,500 photon beams and 81,000 proton beamlets. Data format and usage notes: Data are organized into photon and proton subsets with paired CT-MRI images, beam-level dose distributions, and JSON beam configuration files. Files are provided in compressed MetaImage (.mha) format. The dataset is released under CC BY-NC 4.0, with training data available from April 2026 and the test set withheld until March 2030. Potential applications: The dataset supports benchmarking of fast dose calculation methods, including beam-level dose estimation for photon and proton therapy, MRI-based dose calculation in MRI-guided workflows, and real-time adaptive radiotherapy.

==> acronyms.tex <==
\DeclareAcronym{mc}{
	short = MC ,
	long  = Monte Carlo
}

\DeclareAcronym{gpu}{
	short = GPU ,
	long  = graphics processing unit
}

\DeclareAcronym{pet}{
	short = PET ,
	long  = positron emission tomography
}

\DeclareAcronym{ct}{
	short = CT ,
	long  = computed tomography
}

\DeclareAcronym{lstm}{
	short = LSTM ,
	long  = long short-term memory
}

\DeclareAcronym{rnn}{
	short = RNN ,
	long  = Recurrent Neural Network
}

\DeclareAcronym{cpu}{
	short = CPU ,
	long  = central processing unit 
}

\DeclareAcronym{bev}{
	short = BEV ,
	long  = beam's eye view
}

\DeclareAcronym{rsp}{
	short = RSP ,
	long  = relative stopping power
}

\DeclareAcronym{tps}{
	short = TPS ,
	long  = treatment planning system
}

\DeclareAcronym{mse}{
	short = MSE ,
	long  = mean squared error
}

\DeclareAcronym{rms}{
	short = RMSE ,
	long  = root mean square error
}

\DeclareAcronym{sd}{
	short = SD ,
	long  = standard deviations
}

\DeclareAcronym{mri}{
	short = MRI ,
	long  = magnetic resonance imaging
}

\DeclareAcronym{mr-linac}{
	short = MRI-linac ,
	long  = magnetic resonance imaging-linear accelerator
}

\DeclareAcronym{mlc}{
	short = MLC ,
	long  = multileaf collimator
}

\DeclareAcronym{dl}{
	short = DL ,
	long  = deep learning
}

\DeclareAcronym{ac}{
	short = AC ,
        short-plural = ACs , 
	long  = air cavity ,
        long-plural = air cavities 
}

\DeclareAcronym{bSSFP}{
	short = bSSFP ,
	long  = balanced steady state free-precession,
}

\DeclareAcronym{hu}{
	short = HU ,
	long  = Hounsfield Unit
}


\DeclareAcronym{dir}{
	short = DIR ,
	long  = deformable image registration,
}

\DeclareAcronym{ptv}{
	short = PTV ,
	long  = planning target volume
}

\DeclareAcronym{dsc}{
	short = DSC ,
	long  = Dice similarity coefficient
}

\DeclareAcronym{dvh}{
	short = DVH ,
	long  = dose volume histogram
}

\DeclareAcronym{bce}{
	short = BCE ,
	long  = binary cross-entropy
}

\DeclareAcronym{ere}{
	short = ERE ,
	long  = electron return effect
}

\DeclareAcronym{oar}{
	short = OAR ,
	short-plural-form = OARs ,
	long  = organ at risk ,
	long-plural-form = organs at risk
}

\DeclareAcronym{vmat}{
	short = VMAT ,
	long  = volumetric modulated arc therapy
}

\DeclareAcronym{impt}{
	short = IMPT ,
	long  = intensity modulated proton therapy
}

\DeclareAcronym{rt}{
	short = RT ,
	long  = radiotherapy
}

\DeclareAcronym{mu}{
	short = MU ,
	long  = monitor unit
}

\DeclareAcronym{iaea}{
	short = IAEA ,
	long  = International Atomic Energy Agency
}

\DeclareAcronym{sct}{
	short = sCT ,
	long  = synthetic CT
}

